Remarks on Jurdzinski and Lorys' proof that palindromes are not a Church-Rosser language

In 2002 Jurdzinski and Lorys settled a long-standing conjecture that palindromes are not a Church-Rosser language. Their proof required a sophisticated theory about computation graphs of 2-stack automata. We present their proof in terms of 1-tape Turing machines.We also provide an alternative proof of Buntrock and Otto's result that the set of non-square bitstrings, which is context-free, is not Church-Rosser.

==> midbit.tex <==
\newcommand{\leftend}{~{\overline{\$}}~}
\newcommand{\rightend}{~\$~}
\newcommand{\halved}{\mbox{\rm packed}}
\newcommand{\ohalved}{\overline{\mbox{\rm packed}}}
\newcommand{\odd}{\mbox{\rm odd}}
\newcommand{\even}{\mbox{\rm even}}


$$ \midbit = \{ u0v \in \{0,1\}^*:~ |u|=|v| \}$$ is
the set of bitstrings with 0 in the middle.  We
have mentioned that it is not congruential. Also,

\begin{lemma}
\label{lem: midbit not dcfl}
$\midbit$ is not a DCFL.
\end{lemma}

{\bf Proof.}  We apply the pumping lemma from
[\ref{yu}].  Let
$$ x= 1^n 0 1^{n-1},\quad y=1, \quad z=101^{2n+1},
w = xy = 1^n 0 1^n,\quad w' = xz = 1^n01^n01^{2n+1}.$$ Both
$w$ and $w'$ are in $\midbit$.  By the pumping lemma [\ref{yu}],
if $n$ is sufficiently large, there are two possibilities
for `pumping.' Either

\begin{itemize}
\item
we can replace $x=rstuv$ by $rtv$ where $su\not=\lambda$
and $rtvz \in \midbit$. This is false since
the middle bit in $rtvz$ is among the rightmost ($2n+1$)
1-bits,
or
\item
$x$ contains a substring $t$ near its right-hand
end, and  $y$ contains a substring $u$, such
that $t$ and $u$ can be pumped simultaneously in
$x$ and $y$.  However, if $n$ is large then
$t$ is to the right of the zero in $xy$, and
pumping $t$ and $u$ produces strings not
in $\midbit$. {\bf Q.E.D.}
\end{itemize}


But $\midbit$ is a Church-Rosser language, as we show
by exhibiting a Church-Rosser Thue system $T$ which
isolates the middle bit of odd-length bitstrings.

Given an odd-length bitstring $w$, let $w_1$ be the first, third, fifth,
\ldots bits of $w$, and let $w_2$ be the second, fourth, \ldots
bits. If $|w|\bmod 4 = 1$, then $|w_1|$ is odd and the middle bit of $w$ is
the middle bit of $w_1$; otherwise, it is the middle
bit of $w_2$.  Based on this observation, one can
exhibit a shrinking deterministic
2-stack automaton accepting $\midbit$
which shows that $\midbit$ is Church-Rosser
[\ref{bo},\ref{no}].  However we describe
in outline a specific Thue system $T$, as a curiosity,
and to show that it is large (20,720 rules).




We shall use $t_1=\leftend $ and $t_2=\rightend$ to provide
the necessary context.


The string to be reduced will therefore be written as

$$ x= \leftend  a_1 a_2 \ldots a_n \rightend $$ and we require
that if $n$ is odd then 
$$\leftend x \rightend \redstar_T \leftend  a_{n/2+1}\rightend$$
and if $n\geq 2$ is even then the irreducible string
in $[x]_T$ has length at least 4 (also $\leftend \rightend$ is irreducible,
$n=0$).

The alphabet of $T$ will also include
barred and unbarred {\em double symbols}
$~\overline{[b_1 b_2]}, [b_1b_2]$, $b_1,b_2 = 0,1$,
and {\em sweep symbols} $~\overline{P},Q,R,~\overline{Q},
~\overline{R}$.  For a barred or unbarred double symbol
$$ ~\overline{[b_1b_2]},\quad [b_1b_2],$$ the
{\em odd side} (bit) is $b_1$ and the {\em even side} is $b_2$.

{\bf The first $208$ rules of $T$, whose redexes involve bitstrings.}
In the description below, $b_1, b_2 \ldots$ are single bits.

\begin{itemize}
\item
The first 40 rules apply to strings $\leftend x \rightend$ where
$x$ is a bitstring of length $\leq 5$. If $|x|=1$ or $|x|$ is even
and $|x|<5$, $\leftend x \rightend$ is
irreducible. Otherwise
\begin{eqnarray*}
 \leftend  b_1 b_2 b_3  \rightend \to \leftend  b_2  \rightend  \\
 \leftend  b_1 b_2 b_3 b_4 b_5  \rightend \to \leftend  b_3  \rightend
\end{eqnarray*}

\item
The next 64 rules initiate a right-sweep by packing
the first 4 bits into two double symbols and introducing
the right sweep symbol $\overline{P}$.
$$
 \leftend  b_1 b_2 b_3 b_4 b_5 b_6 \to
~\overline{ [ b_1 b_2 ] } ~
~\overline{ [ b_3 b_4 ] } ~\overline{P}~ b_5 b_6 
$$
\item
The next 64 rules continue the right sweep by packing and shifting.
$$
 ~\overline{P}~ b_1 b_2 b_3 b_4 b_5  b_6 \to
~\overline{ [ b_1 b_2 ] } ~
~\overline{ [ b_3 b_4 ] } ~
~\overline{P}~ b_5 b_6
$$
\item
The next 40 rules terminate a right sweep and initiate
a left sweep.
\begin{eqnarray*}
 ~\overline{P}~ b_1 b_2 b_3 b_4 b_5  \rightend \to
~\overline{ [ b_1 b_2 ] } ~
~\overline{ [ b_3 b_4 ] } ~
~\overline{ [ b_5 0 ] }~Q \rightend  
\\
 ~\overline{P}~ b_1 b_2 b_3  \rightend \to
~\overline{ [ b_1 b_2 ] } ~R \rightend  
\end{eqnarray*}
\end{itemize}

{\bf Notation:} $\odd([b_1b_2])=\odd(\overline{[b_1b_2]})=b_1,$ the odd side
of double symbols; similarly $\even$.  These are homomorphisms,
so $\odd([a_1a_2][a_3a_4]) = a_1a_3$, etcetera. If
$x = a_1 a_2 \ldots a_n$ is a bitstring and $n$ is even,
then $\halved(x) = [a_1 a_2] \ldots [a_{n-1} a_n]$.  If
$\alpha$ is any string and $r\leq |\alpha|$, then $\alpha^{[r]}$ is its
prefix of length $r$.

\begin{lemma}
\label{lem: reductive properties of T}
Given $x\in \{0,1\}^*$, 
if $|x| \leq 5$ then the
above rules reduce $x$ to $\leftend b \rightend$
if and only if $x$ is odd and $b$ is its middle bit.

If $|x|\geq 5$ is even, then the above rules
reduce $\leftend x \rightend$
to an irreducible string containing $\overline{P}$.

If $|x| = 4k + 5$, then the above rules reduce
$\leftend x \rightend$
to $\leftend \ohalved(x0) Q \rightend$, and the middle
bit of $x$ is the middle bit of $\odd(\ohalved(x0))$.

If $|x| = 4k + 3$, then the above rules reduce
$\leftend x \rightend$ to
$\leftend \ohalved (x^{[4k+2]}) R\rightend$,
and the the middle bit of $x$ is the 
middle bit of $\even(\ohalved(x^{[4k+2]}))$.\qed
\end{lemma}

The remaining rules of $T$ are as follows.
(For the sake of brevity, $\alpha = \alpha_1 \ldots \alpha_6$
is a string of 6 double symbols,
$\beta$ is a string of 5 double symbols, and $\gamma$
is a string of $3$ double symbols.  Also
$\overline{\alpha}$ is a string of 6 barred double symbols,
etcetera.)

\begin{eqnarray*}
\overline{Q}\alpha \to \ohalved(y)\overline{Q}
\alpha_5 \alpha_6, \qquad y = \odd(\alpha^{[4]})\\
\overline{Q}\beta\rightend \to
\ohalved(y0) Q\rightend,\qquad y = \odd(\beta)\\
\overline{Q}\overline{\gamma}\rightend \to
\ohalved(y^{[2]}) R\rightend,\qquad y = \odd(\gamma)\\
\leftend \overline{Q} [b_1 b_2] \rightend \to \leftend b_1 \rightend
\end{eqnarray*} Rules involving $\overline{R}$ are similar,
except they work with the even part of double symbols.

It remains to mention the `right-to-left sweep' rules involving
$Q$ and $R$.  They are mirror-images of the above rules.
For every rule $X\to Y$ involving $\overline{Q}$ or $\overline{R}$,
there is a rule $\overline{X}^R\to\overline{Y}^R$ involving
$Q$ or $R$; that is, both sides are reversed,
and barred symbols exchanged with the corresponding
unbarred symbols.  

Following the ideas of Lemma \ref{lem: reductive properties of T},
one can prove that the above rules do reduce
$\leftend x \rightend$ to $\leftend b \rightend$ if and
only if $|x|$ is odd and $b$ is its middle bit.

\begin{lemma}
$T$ is Church-Rosser.
\end{lemma}

{\bf Sketch proof.} No two rules have the same redex,
so it is enough to show that redexes do not overlap
[\ref{bo}].
Every redex is of the form
$\overline{U}V$ where $\overline{U}$ is a nonempty
string of barred symbols and $V$ is a nonempty string
of unbarred symbols.  Hence if two redexes overlap,
their overlap must include the rightmost barred symbol
and the leftmost unbarred symbol.

Redexes in the first 104 rules do not contain
a `sweep symbol' $\overline{P},\overline{Q},\overline{R},Q,R$,
and the only barred symbol they have is $\leftend$, so
if they overlap then they are identical.

Redexes in the other rules contain a `sweep symbol'
so if two overlap, they involve the same `sweep symbol' and
must be identical.\qed

